WEIRD ICWSM: How Western, Educated, Industrialized, Rich, and Democratic is Social Computing Research?

Much of the research in social computing analyzes data from social media platforms, which may inherently carry biases. An overlooked source of such bias is the over-representation of WEIRD (Western, Educated, Industrialized, Rich, and Democratic) populations, which might not accurately mirror the global demographic diversity. We evaluated the dependence on WEIRD populations in research presented at the AAAI ICWSM conference; the only venue whose proceedings are fully dedicated to social computing research. We did so by analyzing 494 papers published from 2018 to 2022, which included full research papers, dataset papers and posters. After filtering out papers that analyze synthetic datasets or those lacking clear country of origin, we were left with 420 papers from which 188 participants in a crowdsourcing study with full manual validation extracted data for the WEIRD scores computation. This data was then used to adapt existing WEIRD metrics to be applicable for social media data. We found that 37% of these papers focused solely on data from Western countries. This percentage is significantly less than the percentages observed in research from CHI (76%) and FAccT (84%) conferences, suggesting a greater diversity of dataset origins within ICWSM. However, the studies at ICWSM still predominantly examine populations from countries that are more Educated, Industrialized, and Rich in comparison to those in FAccT, with a special note on the 'Democratic' variable reflecting political freedoms and rights. This points out the utility of social media data in shedding light on findings from countries with restricted political freedoms. Based on these insights, we recommend extensions of current "paper checklists" to include considerations about the WEIRD bias and call for the community to broaden research inclusivity by encouraging the use of diverse datasets from underrepresented regions.

==> sections/notes.tex <==
% benefits.. raise these in the discussion
% posters are more inclusive

% shadowing of people in less represented countries help how to write
% reinforce/embrace
% how to target money in certain universities like the bill gates foundation.. tackle global problems. 

% Theoretical: growing body of literature about WEIRD studies. we provide empirical evidence in a conference proceedings that is dedicated to social media.. social media is full of biases, and yet the community is less WEIRD compared to HCI ML communities.

% Practical: 
% - Extend the current checklist. praise them that is a good thing but include more questions. expand section 5 of the checklist and include specific questions or a score how weird is the paper before submission. we can create a website where authors can submit the details of their dataset and get a score.

% - responsible AI statement.. praise again neurips, icml, alexandra's work.. more on harms and risks of using these datasets from specific countries


% - open-source platform for encouraging authors to share their data and create standard benchmarks to cover, if possible, the whole world.

% - champion author diversity. encourage collaborations across authors. for dataset and poster papers, create shadow mentoring programs to enable new researchers or those from under-represented groups to publish in the main proceedings (shadowing opportunities by senior members in the community). continue doing that.. praise them.


% future work
% It would be interesting to explore the impact of these diversity issues in the context of Fairness, Accountability, and Trust. For example, it would be interesting to read about the intersection between AI algorithms and legislative action perspectives, public perceptions and the use of AI in public administration in WEIRD countries, or the potential impact of the absence of rigorous scholarship on these questions for countries outside of WEIRD society. (See: "Artificial Intelligence: the global landscape of ethics guidelines (2019)" or "A Global South perspective for ethical algorithms and the State (2023)".

% because the overfocus on the Egnlish language implies non-English speaking countries are less represented than what penetration rates would suggest.


% shadowing opportunities by senior members in the community
% -DISCUSSION. recommends more multinational author teams, which appear to correlate with less “WEIRD” data and results.
% -DISCUSSION.  remove reproducibility? I don’t readily see how reproducibility could alleviate the weirdness of the samples if the problem originates in the selection of the samples.
 
% -LIMITATION. WEIRD samples do not necessarily mean a lack of diversity in perspectives.  I emphasize this because in a different scenario for example when we look at work in development economics, if you look at the samples used (as in this submission) they would be overwhelmingly coming from the global south, and you could conclude the field is not WEIRD at all. But if you look at the authors, their institutions and training, and their methods used and interpretations of the results and so on, these factors could still be heavily western influenced. In the past, there are works at FAccT and CHI discussing various counter-algorithm movements (e.g #FuckTheAlgorithm: algorithmic imaginaries and political resistance) or trying to understand the societal impact of algorithms from different perspective (e.g. An Action-Oriented AI Policy Toolkit for Technology Audits by Community Advocates and Activists). Granted that they are situated in the western contexts, I think the draft could benefit from the authors discussing more future directions that aim at looking at the perspectives represented in addition to demographics and cultural contexts. The authors could also discuss looking at more nuanced views within the western countries represented by immigrants, lower-income populations, cultural minorities and so on.
 
% - FUTURE WORK.  it would be interesting to read about the intersection between AI algorithms and legislative action perspectives, public perceptions and the use of AI in public administration in WEIRD countries, or the potential impact of the absence of rigorous scholarship on these questions for countries outside of WEIRD society. (See: "Artificial Intelligence: the global landscape of ethics guidelines (2019)
